AI Research Considerations for Human Existential Safety (ARCHES)

Framed in positive terms, this report examines how technical AI research might be steered in a manner that is more attentive to humanity's long-term prospects for survival as a species. In negative terms, we ask what existential risks humanity might face from AI development in the next century, and by what principles contemporary technical research might be directed to address those risks. A key property of hypothetical AI technologies is introduced, called \emph{prepotence}, which is useful for delineating a variety of potential existential risks from artificial intelligence, even as AI paradigms might shift. A set of \auxref{dirtot} contemporary research \directions are then examined for their potential benefit to existential safety. Each research direction is explained with a scenario-driven motivation, and examples of existing work from which to build. The research directions present their own risks and benefits to society that could occur at various scales of impact, and in particular are not guaranteed to benefit existential safety if major developments in them are deployed without adequate forethought and oversight. As such, each direction is accompanied by a consideration of potentially negative side effects.

==> buffer.tex <==
%
For instance:


		On the other hand, there are some ways in which  cooperation in the governance of powerful AI systems could be particularly beneficial from an existential safety perspective, elaborated below.  Moreover, there may be design choices in the development of AI technology that could make the potential pitfalls of cooperative governance less likely.  The present objective, \emph{\bbcgt}, is to develop AI technology and accompanying governance procedures to ensure that the cooperative governance of powerful AI technologies would be beneficial from a broad variety of perspectives, including but not limited to existential safety.

% technology outpacing

\begin{quote}
 ``it was far from clear, even to the finest
of contemporary military minds, what the transformation of infantry firepower meant for
logistics, organization, doctrine, tactics, operations, strategy and even high policy (not
that the final item generally was considered a proper military concern).''
-- War, Peace, and International_Relations


\end{quote}

	% alignment


			\emph{Alignment for Advanced Machine Learning Systems (AAMLS)} \citep{taylor2016alignment} examines the question, ``As learning systems become increasingly intelligent and autonomous, what design principles can best ensure that their behavior is aligned with the interests of the operators?''  As such, the concept of ``preference alignment'' in this research agenda corresponds roughly to the notion of ``alignment'' as used by \citet{taylor2016alignment}.  We defer the reader to AAMLS for the alternative perspectives developed therein.







% biases:
% unrecognized prepotence:

Moreover, a number of systematic human biases that are well-replicated in the psychology literature might play a role in a failure to intuitively recognize \prepotence:

\begin{itemize}
	\bias{Scope insensitivity} is the tendency for intuitive human judgments to be insensitive to orders of magnitude.  This insensitivity has been observed repeatedly in numerous studies specifically on intuitive valuations of benefits to large numbers of people, so-called ``public goods'' \citep{erick1998scope,carson1997contingent,veisten2004scope,hsee2004music}.
	Since existential risk reduction is a public good, we should expect reasoning about it to be scope insensitive by default.
	Thus, absent a technically rigorous approach to evaluating both the impact and the likelihood of \prepotent and/or MPAI systems, these risks are liable to be either overestimated or underestimated, with cases of under-estimation leading to greater \xrisks.\footnote{It is interesting to note that scope insensitivity could also lead to the underestimation of potential benefits from technological advancements.  However, the underestimation of benefits does not currently appear to be a limiting factor in AI development, perhaps because AI researchers are currently well-funded and generally optimistic about the benefits of their work.
	It is in part for this reason that the present document is focused on downside risk mitigation.}

	\bias{Illusion of control} is a human bias defined as ``an expectancy
	of a personal success probability inappropriately higher than the objective
	probability would warrant'' \citep{langer1975illusion}.
	Since 1975, a rich literature has examined the presence of illusory control in a variety of circumstances; see \citet{presson1996illusion} for a meta-analysis of 53 experiments from 29 articles.
	Since \prepotence  of an AI system by definition constitutes a loss of human control, the illusion of control effect is extremely pertinent.

			\end{itemize}

% unrecognized misalignment:
Aside from being a poor practice for high-stakes engineering work, reliance upon intuitive judgments about alignment could render developers susceptible to any number of long-observed and well-replicated cognitive biases, including:
			\dksays{minor: the stuff about "intuitive judgments/interpretation" echoes the previous section and is a bit redundant.  We could say "as in [the previous section], or try and compress the two a bit.}

In any case, a rigorous scientific theory and practice of intelligence alignment is needed to displace what would otherwise be ad hoc, intuitive judgments about alignment.


			\begin{itemize}

				\bias{Illusion of control.} See \risknum{urprep}.
				\bias{Scope insensitivity.} See \risknum{urprep}.

				\bias{Escalation of commitment,} also known as the ``sunk cost fallacy'', the tendency of groups and individuals to escalate commitment to a failing course of action has been examined by a rich literature of management and psychological studies; see \citet{staw1981escalation} and \cite{brockner1992escalation} for literature reviews.
				Unfortunately, software development teams in particular appear to be prone to escalating commitments to failed approaches \citep{keil2000cross}.
				The escalation of commitment effect contributes to the risk that an AI development team, having designed a system that will be \prepotent and difficult to align, might continue to pursue the same design instead of pivoting to a safer approach.
				%\todo\bias{Moral self-licensing} This is highly pertinent if an AI development team develops a powerful system that they are excited to deploy, and they view safety measures as an obligation rather than an intrinsically rewarding pursuit.
				%Such a group might feel justified in deploying in deploying an unsafe system because of previous of failed attempts to make it safer.
				% Meta-analysis showed small effect size: https://www.researchgate.net/profile/Marcel_Zeelenberg/publication/272837497_A_Meta-Analytic_Review_of_Moral_Licensing/links/552253ad0cf2f9c13052a936/A-Meta-Analytic-Review-of-Moral-Licensing.pdf

				\bias{The mere-exposure effect} is the psychological tendency for continued exposure to a stimulus to cause, in most people, an increase in positive affect toward that stimulus.
				This effect was found to be robust and reliable by a meta-analysis of 208 independent experiments between 1968 and 1987 \citep{bornstein1989exposure}.
				If the developers of a powerful AI system fall prey to the mere-exposure effect, their experience with the system throughout its development process could bias them toward believing it is safe for deployment.

				For meta-analyses of this phenomenon, see \citet{klein2002perceived} and \citet{brewer2007meta}; for a neurological account, see \citet{sharot2007neural}.


				\bias{Optimism bias} is the general tendency for most people to believe that they are less at risk than their peers for many negative events, such as getting cancer, becoming alcoholics, getting divorced, or getting injured in a car accident.
				This sort of self-centered optimism could create a feeling
				that any given global catastrophe might harm everyone else, ``but not me'', hence leading to a
				systematic underestimation of probabilities like $P(\mathrm{extinction}\mid \mathrm{catastrophe})$ and $P(\mathrm{misalignment}\mid \mathrm{prepotence})$.  As a result, persons in positions of responsibility for near-prepotent AI systems might be more careless than we'd like when it comes to potential global catastrophes.
			\end{itemize}

			Presumably there exist other systematic errors and biases that would interfere with intuitive assessments of experiments to ascertain the alignment of a powerful AI system.  Indeed some biases could go in the other direction, yielding too little trust in technology, but such errors are not the focus of this agenda.


\section{Supplemental remarks}\label{sec:remarks}
\acsays{I'm inclined to remove this section unless all of SR, JF, and DK think we should keep it.}
Here we include a little more non-technical content that was not necessary to include before the research directions, but nonetheless seemed worth sharing afterward.
            \dksays{use of "we"/"us"/"our"}

	\subsectiondef{timingsocial}{Timing and social considerations}
		\fl{3}
			The relative impacts on existential risk of the research \directions in this document depend significantly on external factors that influence the order and manner in which future technologies will be developed and implemented.
			Here we outline several timing and social considerations that we believe are important for researchers to examine when deciding whether and how to prioritize existential safety as an objective in their work.
            \dksays{use of "we"/"us"/"our"}

			\paragraph{Backward-first vs forward-first prioritization.}
            \dksays{moderate: this paragraph doesn't seem to fit with the title of this subsection}
			One way to prioritize research directions for existential risk reduction is by backward induction, i.e., reasoning backward from future risk scenarios to potentially relevant present-day research contributions.  However, in order to realistically predict and control the impact of one's research, one should augment this backward-induction perspective with forward-induction.  This means reasoning forward from the
			potential present-day research contributions to identify the many positive and negative ways a given research contributions could be applied, aside from the motivating future use-case.

			We call this combination of reasoning ``backward-first'' prioritization.  For instance, one could reason as follows:

			\begin{enumerate}
				\item (starting to think about the future) Someday someone might accidentally release a misaligned prepotent system without realizing it.
				\item (reasoning backward from the future) Therefore, we should improve methods today for aligning powerful systems with human values.
				\item (reasoning forward from the present) Assuming we develop such alignment methods, we should ensure the alignment methods are not abused by careless or malicious actors.
			\end{enumerate}

			This style can be contrasted with what one might call ``forward-first'' prioritization, which looks more like this:

			\begin{enumerate}
				\item (starting to think about the present) I have some ideas for how to cause AI systems to understand what humans want.
				\item (reasoning forward from the present) This research could be used for personal assistant software, or maybe later for directing more powerful AI systems that could pose risks to society.
				\item (reasoning backward from the future) We should make sure that whatever framework we use is sufficient to model risk aversion, e.g., using a utility function to score potential outcomes.
			\end{enumerate}

			\noindent (These styles can be combined, and even concatenated.)

			The research directions in ARCHES were generated primarily from backward-first prioritization, in part because backward-first thinking appears to us to be relatively neglected relative to forward-first thinking in the way researchers prioritize their work.

			\paragraph{Time-ordering influences the relative priority of risks.}
			Whether using forward-first or backward-first prioritization, during the ``reasoning backward from the future'' step, one can also ask:
			\begin{itemize}
			\item How important is the future problem I'm imagining solving?
			\item How urgently will the solution be needed, once the problem arises?  And,
			\item Does there appear to be enough time between now and the future problem for me and others to implement a solution?
			\end{itemize}

			By asking such questions, timing and social considerations can be given an opportunity to affect one's assessment of the relative importance and urgency of various research directions.  For instance:

			\begin{itemize}
				\item If one believes carelessness is sufficiently more common among AI developers than malice or indifference, an argument surfaces that \risksref{voldep} are less likely to obtain than other \risksref{mpais}.
				On the other hand, if one believes established institutions will be effective and well-coordinated in their own commitments to long-term public safety, but ineffective in preventing terrorism, warfare, or public recklessness, this presents an argument that \risktitle{voldep} may be a relatively more pressing concern.
				\item If one expects that business executive and political leadership roles may be occupied by AI systems well before \prepotent AI systems exist, there is reason to believe \risksref{races} and \risksref{econ} are more urgently important than specific \risktitle{mpais}.
				On the other hand, if one believes \prepotent AI systems will exist before the widespread adoption of human-level AI in roles of economic or political leadership, there is reason to be more directly concerned about \risktitle{mpais} rather than \risktitle{hazsoc}.

				\item If one expects leading AI development teams to be sufficiently individually concerned with safety, at least relative to their mistrust of the deployment decisions that other teams would make, then there is reason to prioritize generalized efforts to avert  \risksrefs{uncdev,invdep,races} over targeted efforts to avert other \risksref{mpais}.  On the other hand, one could believe that some \risktitle{mpais} will be likely to occur before \risktitle{races} will have a chance to take place, or that research on multi/single delegation will have insufficient time to affect culture prior to the imminence of such race dynamics.  This would reduce the relative importance of multi/single delegation research for x-risk reduction.
			\end{itemize}

			To any researcher who is considering making existential safety a major objective in their own research priorities, we would suggest spending at least 3\% of your research time engaged in detailed reflections of this sort, with attention to both timing and social considerations.  This sort of reasoning can lead one to develop research ``timelines'' in one's thinking, like ``Within $X$ or so years I expect problem A to arise and become urgent.  And, it might take $2X$ years for the research community to develop a solution for it.  So, I want to focus my attention on helping other researchers to notice and understand this, and take my best shot at helping to solve it before the solution is urgently needed.''
            \dksays{use of "we"/"us"/"our"}

			The present authors have explicitly decided \emph{not} to argue in this document for belief in any particular research timelines, because doing so would greatly lengthen and complicate our discussion.  However, we do in fact have opinions in mind, and wish to encourage other researchers to develop views of their own on these questions, not only over short conversations at conferences or social gatherings, but through detailed and collaborative analyses.

			\paragraph{Short timelines preclude flow-through effects.}
			Some research objectives, such as \dirref{humancognitive} and \dirref{boun}, have a large number of flow-through effects on the other research \directions in ARCHES, and therefore on longer time scales these priorities could have a comparatively large impact.
			On the other hand, if the time until a risk will manifest is too short, longer chains of potential impact may not have time to take effect on the world.

			\paragraph{Anticipating responsiveness may lead to unresponsiveness.}
			When thinking about the future and what problems might arise in it,
			it is tempting to assume that any scenario that would pose a significant risk of destroying the human species would be too foolish a mistake for anyone to allow it to happen, and that therefore no research is needed to prepare for such scenarios.
			However, if the prevalence of this argument in the minds of leaders and intellectuals prevents their wisdom from coming to bear on avoiding these risks, then the argument becomes invalid.
			That is to say, anticipating responsiveness can lead to unresponsiveness.  For, suppose too many researchers treat concerns about an existential risk scenarios as over-reactions on the grounds that someone else will address the issue.  If as a result no one addresses the issue, we will end up back in a bystander-effect-like situation where a catastrophe can manifest and everyone will be surprised that no one else took measures to avert it.

			\paragraph{Overreaction can lead to underreaction.}  On the other hand, if at some point everyone believes that no one else is doing anything about existential risk, this could lead to a lot of redundant and/or inefficient actions being taken that might even undo one another.  The solution to avoiding both underreactions and overreactions is likely to maintain in common knowledge an understanding of how much and what quality of research effort is being directed at various areas of existential risk reduction, so that trust is maintained across decades and generations that existential risk is a topic that humanity treats responsibly.

			\paragraph{Reflections on branding.}
			Given that overreactions can lead to underreactions, we considered a number of alternative titles have been suggested for the  present document that would reference existential risk less explicitly, and therefore perhaps evoke fewer negative reactions. However, in the long run, it seems important to be able to discuss human survival as an explicit technical objective, and using less direct language encumbers that discussion.  So, in the end, we settled on an explicit and sober discussion of existential risk as our guiding theme, and on including the term ``existential'' in our title.  Below are some examples of terminology that were considered but not adopted in the title of this agenda, due to being either too general or too specific:
            \dksays{use of "we"/"us"/"our"}

			\begin{itemize}
				\item ``AI safety'' is a broadly useful term, which naturally admits AI existential safety as a special case.   Indeed, many techniques from present-day AI safety, such as autonomous vehicle navigation, might be transferrable to lowering AI x-risk.

				However, students and researchers interested in AI x-risk have been observed to confuse one another when using ``AI safety'' as a euphemism for more specific concerns about human survival.  For instance, the self-replication of AI systems is not a concern in most domains of AI safety, nor is the strategic overpowering of a human attempting to gain access to an AI system's ``off switch'' \citep{hadfield2016off}.  Conflating these latter concerns with other AI safety topics leads to confusion in the peer review process and bewildered conference attendees struggling to imagine a Roomba cleaning robot that somehow disables its off-switch mechanism.
                %\dksays{minor: TODO: rephrase: "overpowering" sounds a bit odd.  Also, we can mention SIDS, and a few other related works...}

				\item ``Long-term AI safety'' has the advantage that it is less likely to be confused with safety for AI systems existing in 2019, and allows one to ask important questions like ``What techniques from autonomous vehicle safety might generalize to long-term AI safety?''  However, if researchers must always refer to existential risks as ``long term'' risks, and a more immediate existential risk arises at some point, it will be difficult to discuss until researchers get around to saying ``AI x-risk'' or something else that refers more directly to the problem at hand.

				\item ``Artificial general intelligence (AGI) safety'' has the advantage that present-day AI systems are not ``generally intelligent'', so again the topic cannot be confused with safety for 2019-level AI technologies.  However, as we argue in \refsec{key}, ``general intelligence'' is not a necessary condition for an AI system to pose an existential risk.  Moreover, if researchers are only able to easily discuss risks that would arise from AGI, then existential risks arising from narrower capabilities---which could arise sooner---will remain neglected.
            \dksays{use of "we"/"us"/"our"}
			\end{itemize}

	\subsection{Sobriety versus sensationalism in discourse}
		\fl{3}
			Existential risk is for many people an uncomfortable topic to discuss, because it is both frightening and grandiose.  Some might argue that therefore it should not be discussed at all.  This, of course, would be a highly irresponsible position to take from a global perspective: we cannot take precautions against risks that we cannot discuss.  However, the fact that existential risks can be upsetting means that it can be sensationalized, which presents an important challenge for discourse.  This challenge is deserving of some explicit and shared reflection.

			First, consider that the help of popular writers and communicators will likely always be needed to educate society about the nature of AI technology and the risks and benefits that accompany it.  Indeed, in recent years there have been a growing number of news articles written about existential risks from AI.

			However, it seems to the present authors that in many of these articles, nuance has been sacrificed for sensationalism.  Whether intentionally or unintentionally, the natural pull and selection mechanisms of public discourse
			seems to often result in the misrepresentation of carefully laid out arguments---such as those in \emph{Superintelligence} \citep{bostrom2014superintelligence}---in favor of attention-grabbing headlines.
			Such sensationalism can damage the credibility of sound arguments in the eyes of potential collaborators and policymakers.
			Indeed, if existential safety is sensationalized, even professional AI researchers discussing it at conferences will struggle to express their more nuanced perspectives on it to one another, as those views will too often be mistaken for their nearest sensationalized variants.  To an extent, this problem already exists.

			This pattern also introduces a dynamic wherein making a professional study of existential safety might be seen as form of attention-seeking.  From a global perspective, one would not hope for all professional AI researchers to avoid the topic of existential safety for fear that they might be seen as seeking attention.  Yet, it is difficult even to express these considerations without somehow accidentally portraying this document as being at the center of some controversy.

			Perhaps a solution, then, would be to explicitly ask public writers and communicators to avoid sensationalizing our work.  Naively, this is certainly our preference.  Indeed, while it might seem that drawing attention to our work would be doing us a favor, if that attention comes at the cost of precision, or with too much focus on problems and not enough focus on potential solutions, the result can be worse than no attention at all.

			But would such a request be fair?  Is sensationalism always bad?  If we were approaching the precipice of a global risk, would sensationalizing it always be the wrong reaction?  And, how is everyone supposed to know when we're at that precipice?

			These are difficult questions that are beyond our expertise, and certainly beyond the scope of this agenda.  We express them so as to profess our ignorance, and to be forthright about the discursive challenge we find ourselves to be facing.
            \dksays{use of "we"/"us"/"our"}

			All of the above considered, it seems to us at the time of writing this agenda that concerns about sensationalization or misinterpretation ought to be outweighed by the intellectual and societal benefits of reasoning and writing in sober detail about existential safety.  Consequently, despite all of the above concerns, this research agenda has sought to be forthright in categorizing potential risks, and how one might begin to address them.

			%\paragraph{Reflections on motivating vs justifying research.}
			%The publishing of this agenda will make it much easier for researchers to cite a document to suggest that their work may be related to existential risk reduction.
			%Indeed, we hope that this will be the case, because of the potential for more targeted collaborations to arise from tangential relationships.
			%In doing so, we ask that researchers think carefully about the distinction between their work being \emph{related} to existential risk reduction versus being \emph{motivated by it}.


			%There an incentive within academia to name the most easily fundable plausible application of a research project as a ``motivation'' for their work, even when it has little bearing on the interest of the scientist conducting the research.
			%In a nascent field like existential risk reduction, following this incentive can have detrimental effects on our collective ability to orient on important problems.  In general, research carried out with a particular goal X in mind (e.g., reducing existential risk) is much more likely to be useful for X than research
			%that claims X as an after-the-fact potential application.  In other words, research actually ``motivated by'' X is more likely to actually help with X that research that is merely ``related to'' X.

			%To argue this important distinction between motivation and relevance, we propose to think of research planning as somewhat akin to motion planning in robotics.
			%The space of potential research \directions is large, and the chance of hitting a target in that space by accident is much lower than the chance of hitting it on purpose.
			%When executing a physical motion plan, small feedback corrections (and occasionally more fundamental replanning) are needed to enable continued progress in spite of the inevitable modeling inaccuracies or unexpected events.
			%For an analogous control mechanism to guide research toward a goal, that goal must be viewed as more than a collateral benefit; it needs to be an integral part of the researcher's decision-making process.
			%Put succinctly, the implicit drives of the researcher matter quite a bit to their long-term trajectory.

			%Therefore, if you wish to cite this agenda as relevant to your work, but no choices were made during the course of your project to retain its applicability to existential risk reduction, and you would have undertaken the same project even if existential risk were not a concern, then we ask that you claim only that your work is ``related to'' or ``relevant to'' this agenda, rather than ``motivated by'' existential risk reduction.  Otherwise, we risk creating a false sense of security in the world, from a false representation of how many people are genuinely pursuing existential risk reduction as a primary intellectual goal.

